Measurements of the $\gamma_{v} p \rightarrow p' \pi^{+} \pi^{-}$ cross section with the CLAS detector for $0.4$ GeV$^{2}$ $< Q^{2} <$ $1.0$ GeV$^{2}$ and $1.3$ GeV $< W <$ $1.825$ GeV

New results on the single-differential and fully-integrated cross sections for the process $\gamma_{v} p \rightarrow p' \pi^{+} \pi^{-}$ are presented. The experimental data were collected with the CLAS detector at Jefferson Laboratory. Measurements were carried out in the kinematic region of the reaction invariant mass $W$ from 1.3 to 1.825 GeV and the photon virtuality $Q^2$ from 0.4 to 1.0 GeV$^2$. The cross sections were obtained in narrow $Q^{2}$ bins (0.05 GeV$^{2}$) with the smallest statistical uncertainties achieved in double-pion electroproduction experiments to date. The results were found to be in agreement with previously available data where they overlap. A preliminary interpretation of the extracted cross sections, which was based on a phenomenological meson-baryon reaction model, revealed substantial relative contributions from nucleon resonances. The data offer promising prospects to improve knowledge on the $Q^{2}$-evolution of the electrocouplings of most resonances with masses up to $\sim$1.8 GeV.

==> qqq <==
\label{intro}
 
\label{fig:e1e_target}
 
\label{fig:zvertex}
 
\label{expt}
 
\label{fig:ec_cut}
 
\label{fig:ph_vs_ph_cc}
 
\label{eq:ineff_zone_cut}
 
\label{fig:ph_el}
 
\label{eq:cc_Poisson}
 
\label{eq:cc_corr_fact}
 
\label{fig:b_vs_p}
 
\label{eq:hadron_hadronmass}
 
\label{fig:elast_pic_position}
 
\label{fig:fid_cuts_neg}
 
\label{fig:fid_cuts_pos}
 
\label{fig:fid_cuts_th_vs_p}
 
\label{fig:qcheck}
 
\label{fig:miss_mass}
 
\label{sec_kin_var}
 
\label{fig:q2vsw}
 
\label{tab:summary_bins}}
 
\label{eq:inv_mass_boundary}
 
\label{eq:bin_width}
 
\label{fig:mass_corr}}
 
\label{cr_sect_formula}
 
\label{fulldiff}
 
\label{flux}
 
\label{polarization}
 
\label{expcrossect}
 
\label{inegr5diff}
 
\label{eff_err}
 
\label{fig:eff_err}
 
\label{efficiency}
 
\label{fig:topologies}
 
\label{rad_corr}
 
\label{radcorrfact}
 
\label{eq_radcorrfact}
 
\label{stat_unc}
 
\label{staterrors}
 
\label{montecarloerror}
 
\label{efferror}
 
\label{errortot}
 
\label{eq:error_stat_mod}
 
\label{fig:sys_err}
 
\label{fig:res_cont}
 
\label{fig:relative_res_cont}
 
\label{fig:e1e_e1c}
 
\label{prev_data}
 
\label{app_a}
 
\label{fig:cr_sec_kinematic2}
 
\label{eq:cr_sec_anglealpha}
 
\label{eq:cr_sec_anglealpha_var}
 
\label{alphavec}\\
 
\label{betavec}\\
 

